Convex and Non-convex Optimization Under Generalized Smoothness

Classical analysis of convex and non-convex optimization methods often requires the Lipshitzness of the gradient, which limits the analysis to functions bounded by quadratics. Recent work relaxed this requirement to a non-uniform smoothness condition with the Hessian norm bounded by an affine function of the gradient norm, and proved convergence in the non-convex setting via gradient clipping, assuming bounded noise. In this paper, we further generalize this non-uniform smoothness condition and develop a simple, yet powerful analysis technique that bounds the gradients along the trajectory, thereby leading to stronger results for both convex and non-convex optimization problems. In particular, we obtain the classical convergence rates for (stochastic) gradient descent and Nesterov's accelerated gradient method in the convex and/or non-convex setting under this general smoothness condition. The new analysis approach does not require gradient clipping and allows heavy-tailed noise with bounded variance in the stochastic setting.

==> Sections/approach.tex <==
\section{Approach}
\label{sec:approach}

In this section, we briefly introduce the high-level idea behind our new approach to gradient-based optimization under the generalized smoothness condition (Definition~\ref{def:smooth_v1}~or~\ref{def:smooth_v2}). To start with, note that Definition~\ref{def:smooth_v2} directly implies the following lemma.

\begin{lemma}
    \label{lem:lsl} If $f$ is $(r,\ell)$-smooth, for any $x\in\cX$ satisfying $\norm{\nabla f(x)}\le G$, we have $\cB(x,r(G))\subseteq\cX$ and for any $x_1,x_2\in \cB(x,r(G))$,
    \begin{align}
    \label{eq:lsl}
    \norm{\nabla f(x_1)\!-\!\nabla f(x_2)}\!\le\! \smcst \norm{x_1\!-\!x_2},\quad f(x_1)\!\le\! f(x_2)\!+\!\innerpc{\nabla f(x_2)}{x_1\!-\!x_2}\!+\!\frac{L}{2}\norm{x_1\!-\!x_2}^2,
    \end{align}
    where $\smcst:=\ell(G)$ is the \emph{effective smoothness constant}.
\end{lemma}
\begin{remark}
     Since we have shown the equivalence between $\ell$-smoothess and $(r,\ell)$-smoothess, Lemma~\ref{lem:lsl} also applies to $\ell$-smooth functions, for which we have $\smcst=\ell(2G)$ and $r(G)=G/\smcst$ if choosing $a=G$ in Proposition~\ref{prop:equ_ass}.
\end{remark}

Lemma~\ref{lem:lsl} states that, if the gradient at $x$ is bounded by some constant $G$, then within its neighborhood with a \emph{constant} radius, we can obtain \eqref{eq:lsl}, the same inequalities that were derived  in textbook analysis \yi{give a reference?} under the standard Lipschitz smoothness condition. With \eqref{eq:lsl}, the analysis for generalized smoothness is not much harder than that for standard smoothness. Since $x$ and $y$ are usually chosen as $x_t$ and $x_{t+1}$ in the analysis, in order to apply Lemma~\ref{lem:lsl}, we need two conditions:  $\norm{\nabla f(x_t)}\le G$ and $\norm{x_{t+1}-x_t}\le r(G)$ for some constant $G$. The latter is usually directly implied by the former for most deterministic algorithms with a small enough stepsize, and the former can be obtained with our new approach that bounds the gradients along the optimization trajectory.

The essential idea of our new approach for bounding gradients can be informally illustrated by the following ``circular'' reasoning. On the one hand, if gradients along the trajectory are bounded by a constant, then based on our discussion above, Lemma~\ref{lem:lsl} can be applied as if standard smoothness condition holds. Then one can basically follow the classical textbook analysis to prove convergence, which implies that gradients converge to zero. On the other hand, any convergent sequence must be bounded. In other words, the bounded gradient condition implies convergence, and convergence also implies the condition back, which forms a circular argument. If we can break this circularity of reasoning in a rigorous way, both the bounded gradient condition and convergence are proved. We will show how to break the circularity by induction for convex functions in Section~\ref{sec:convex} and by contradiction for non-convex functions in Section~\ref{sec:nonconvex}.
